EmbodiedEval: Evaluate Multimodal LLMs as Embodied Agents

Multimodal Large Language Models (MLLMs) have shown significant advancements, providing a promising future for embodied agents. Existing benchmarks for evaluating MLLMs primarily utilize static images or videos, limiting assessments to non-interactive scenarios. Meanwhile, existing embodied AI benchmarks are task-specific and not diverse enough, which do not adequately evaluate the embodied capabilities of MLLMs. To address this, we propose EmbodiedEval, a comprehensive and interactive evaluation benchmark for MLLMs with embodied tasks. EmbodiedEval features 328 distinct tasks within 125 varied 3D scenes, each of which is rigorously selected and annotated. It covers a broad spectrum of existing embodied AI tasks with significantly enhanced diversity, all within a unified simulation and evaluation framework tailored for MLLMs. The tasks are organized into five categories: navigation, object interaction, social interaction, attribute question answering, and spatial question answering to assess different capabilities of the agents. We evaluated the state-of-the-art MLLMs on EmbodiedEval and found that they have a significant shortfall compared to human level on embodied tasks. Our analysis demonstrates the limitations of existing MLLMs in embodied capabilities, providing insights for their future development. We open-source all evaluation data and simulation framework at https://github.com/thunlp/EmbodiedEval.

==> table/main_results_with_affordance.tex <==
% \begin{table*}[h!]
% \centering
% \captionsetup{skip=5pt}
% \caption{Results Overview}
% \label{tab:main_results}
% \renewcommand{\arraystretch}{1.3}
% % \hspace*{-0.5cm}
% \scalebox{0.7}{
% \begin{tabular}{lccccccccccccc cc}
% \toprule
% \multirow{2}{*}{\#Model} & \multicolumn{1}{>{\columncolor{AttrQAColor}}c}{Attr. QA} & \multicolumn{1}{>{\columncolor{SpatialQAColor}}c}{Spatial QA} & \multicolumn{3}{>{\columncolor{NavigationColor}}c}{Navigation} & \multicolumn{4}{>{\columncolor{ObjectInteractionColor}}c}{Object Interaction} & \multicolumn{4}{>{\columncolor{SocialInteractionColor}}c}{Social Interaction} & \multicolumn{2}{c}{\textbf{Overall}} \\
% \cmidrule(r){2-3} \cmidrule(r){4-6} \cmidrule(r){7-10} \cmidrule(r){11-14} \cmidrule(r){15-16}
%  & Succ. & Succ. & Succ. & GcS & SPL & Succ. & GcS & SPL & Afford. & Succ. & GcS & SPL & Afford. & Succ. & GcS \\
% \midrule
% \texttt{Random} & 11.58 & 7.69 & 3.45 & 8.76 & 3.45 & 0.00 & 6.18 & 0.00 & 2.54 & 2.94 & 8.33 & 2.94 & 3.44 & 5.49 & 8.66 \\
% \texttt{Human} & 98.95 & 92.31 & 96.55 & 97.84 & 82.28 & 97.75 & 99.44 & 90.73 & 96.20 & 100.00 & 100.00 & 89.96 & 98.39 & 97.26 & 97.94 \\
% \midrule
% GPT-4o & 37.78 & \textbf{34.00} & \textbf{32.69} & \textbf{45.51} & \textbf{24.19} & \textbf{13.58} & \textbf{24.79} & \textbf{7.34} & 9.41 & 5.88 & 18.63 & \textbf{3.76} & 3.01 & \textbf{26.38} & \textbf{32.93} \\
% GPT-4o-Mini & 31.58 & 15.38 & 27.59 & 39.51 & 15.34 & 2.25 & 17.42 & 1.50 & 9.18 & 5.88 & \textbf{22.06} & 2.98 & \textbf{16.99} & 17.68 & 25.58 \\
% Gemini-Flash & 26.32 & 13.46 & 5.17 & 17.10 & 3.51 & 2.25 & 7.58 & 0.96 & 10.00 & 2.94 & 12.50 & 1.47 & 4.92 & 11.59 & 16.13 \\
% Gemini-Pro & 27.37 & 9.62 & 17.24 & 25.86 & 9.78 & 5.62 & 11.24 & 3.65 & \textbf{10.33} & \textbf{8.82} & 16.91 & 3.41 & 11.11 & 14.94 & 18.83 \\
% Qwen-VL-Max & \textbf{37.89} & 17.31 & 24.14 & 30.03 & 16.87 & 7.87 & 18.54 & 6.15 & 8.10 & 5.88 & 21.32 & 2.65 & 12.75 & 20.73 & 26.27 \\
% Qwen-VL-Plus & 10.53 & 11.54 & 3.45 & 10.49 & 3.45 & 0.00 & 2.43 & 0.00 & 2.96 & 2.94 & 8.82 & 1.68 & 4.84 & 5.79 & 8.31 \\
% \midrule
% InternVL2-Llama3-76B & 17.89 & 15.38 & 13.79 & 24.43 & 13.79 & 1.12 & 8.71 & 1.12 & \textbf{9.56} & 0.00 & 9.80 & 0.00 & 12.90 & 10.36 & 15.32 \\
% InternVL2-40B~\citep{InternVL2} & 14.74 & \textbf{17.31} & \textbf{15.52} & 23.85 & \textbf{15.52} & 0.00 & 7.96 & 0.00 & 5.36 & 0.00 & 12.50 & 0.00 & 7.62 & 9.76 & 14.69 \\
% InternVL2-8B & 13.68 & 13.46 & 8.62 & 18.25 & 4.04 & 0.00 & 7.43 & 0.00 & 3.04 & \textbf{5.88} & \textbf{18.63} & 2.45 & 3.16 & 8.23 & 13.27 \\
% LLaVA-NEXT-72B~\citep{chen2024far} & 16.84 & 3.85 & 10.34 & 20.26 & 10.34 & \textbf{3.37} & 8.61 & \textbf{3.37} & 6.46 & \textbf{2.94} & 12.01 & \textbf{2.94} & 11.25 & 8.54 & 12.65 \\
% LLaVA-OneVision-72B & \textbf{27.37} & 15.38 & \textbf{15.52} & \textbf{28.30} & \textbf{15.52} & \textbf{3.37} & \textbf{10.77} & \textbf{3.37} & 6.21 & \textbf{2.94} & 11.03 & \textbf{2.94} & 4.76 & \textbf{14.33} & \textbf{19.44} \\
% LLaVA-OneVision-7B & 16.84 & \textbf{17.31} & 5.17 & 9.05 & 3.28 & 1.12 & 8.15 & 0.80 & 3.36 & 2.94 & 9.80 & 1.68 & 9.35 & 9.14 & 12.45 \\
% VILA-40B~\citep{lin2024vila} & 18.95 & 7.69 & 5.17 & 12.07 & 5.17 & 1.12 & 5.15 & 1.12 & 6.94 & 0.00 & 7.60 & 0.00 & \textbf{20.37} & 7.93 & 11.03 \\
% VILA-8B & 15.79 & 9.62 & 1.72 & 8.91 & 0.96 & 0.00 & 3.46 & 0.00 & 3.98 & 2.94 & 6.37 & 1.68 & 3.42 & 6.71 & 9.27 \\
% \midrule
% LLaVA-NeXT-Video-32B-Qwen \citep{zhang2024llava} & 21.05 & 7.69 & 6.90 & 14.08 & 5.34 & 0.00 & \textbf{8.61} & 0.00 & \textbf{3.42} & 2.94 & \textbf{12.01} & 0.98 & 4.23 & 8.84 & 13.39 \\
% LLaVA-Video-72B-Qwen2 & \textbf{27.37} & \textbf{9.62} & \textbf{15.52} & \textbf{24.28} & \textbf{9.62} & 1.12 & 8.05 & 0.86 & 2.84 & 0.00 & 9.80 & 0.00 & 7.02 & 12.50 & \textbf{16.95} \\
% Oryx-34B \citep{liu2024oryx} & 18.95 & 3.85 & 5.17 & 13.07 & 4.89 & 1.12 & 7.02 & 1.00 & 2.65 & 0.00 & 8.33 & 0.00 & \textbf{9.09} & 7.32 & 11.33 \\
% VideoLLaMA2-72B \citep{cheng2024videollama} & \textbf{27.37} & \textbf{9.62} & 12.07 & 18.68 & 6.35 & \textbf{2.25} & 7.49 & \textbf{1.38} & 2.30 & \textbf{5.88} & 10.78 & \textbf{2.39} & 3.92 & \textbf{12.81} & 15.91 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

% \begin{table*}[h!]
% \centering
% \captionsetup{skip=5pt}
% \caption{Results Overview}
% \label{tab:main_results}
% \renewcommand{\arraystretch}{1.3}
% \scalebox{0.62}{
% \begin{tabular}{c lccccccccccccc cc}
% \toprule
% \multirow{2}{*}{Category} & \multirow{2}{*}{\#Model} & \multicolumn{1}{>{\columncolor{AttrQAColor}}c}{Attr. QA} & \multicolumn{1}{>{\columncolor{SpatialQAColor}}c}{Spatial QA} & \multicolumn{3}{>{\columncolor{NavigationColor}}c}{Navigation} & \multicolumn{4}{>{\columncolor{ObjectInteractionColor}}c}{Object Interaction} & \multicolumn{4}{>{\columncolor{SocialInteractionColor}}c}{Social Interaction} & \multicolumn{2}{c}{\textbf{Overall}} \\
% \cmidrule(r){3-4} \cmidrule(r){5-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-17}
% % & & \makecell{Succ.\\($\uparrow$)} & \makecell{Succ.\\($\uparrow$)} & \makecell{Succ.\\($\uparrow$)} & \makecell{GcS\\($\uparrow$)} & \makecell{SPL\\($\uparrow$)} & \makecell{Succ.\\($\uparrow$)} & \makecell{GcS\\($\uparrow$)} & \makecell{SPL\\($\uparrow$)} & \makecell{Afford.\\($\uparrow$)} & \makecell{Succ.\\($\uparrow$)} & \makecell{GcS\\($\uparrow$)} & \makecell{SPL\\($\uparrow$)} & \makecell{Afford.\\($\uparrow$)} & \makecell{Succ.\\($\uparrow$)} & \makecell{GcS\\($\uparrow$)} \\

% & & Succ. & Succ. & Succ. & GcS & SPL & Succ. & GcS & SPL & Afford. & Succ. & GcS & SPL & Afford. & Succ. & GcS \\

% \midrule
% \multirow{2}{*}{\makecell[c]{Baseline}} & \texttt{Random} & 11.58 & 7.69 & 3.45 & 8.76 & 3.45 & 0.00 & 6.18 & 0.00 & 2.54 & 2.94 & 8.33 & 2.94 & 3.44 & 5.49 & 8.66 \\
% & \texttt{Human} & 98.95 & 92.31 & 96.55 & 97.84 & 82.28 & 97.75 & 99.44 & 90.73 & 96.20 & 100.00 & 100.00 & 89.96 & 98.39 & 97.26 & 97.94 \\
% \midrule
% \multirow{6}{*}{\makecell{Closed-Source\\Image MLLMs}} & GPT-4o & 37.78 & \textbf{34.00} & \textbf{32.69} & \textbf{45.51} & \textbf{24.19} & \textbf{13.58} & \textbf{24.79} & \textbf{7.34} & 9.41 & 5.88 & 18.63 & \textbf{3.76} & 3.01 & \textbf{26.38} & \textbf{32.93} \\
% & GPT-4o-Mini & 31.58 & 15.38 & 27.59 & 39.51 & 15.34 & 2.25 & 17.42 & 1.50 & 9.18 & 5.88 & \textbf{22.06} & 2.98 & \textbf{16.99} & 17.68 & 25.58 \\
% & Gemini-Flash & 26.32 & 13.46 & 5.17 & 17.10 & 3.51 & 2.25 & 7.58 & 0.96 & 10.00 & 2.94 & 12.50 & 1.47 & 4.92 & 11.59 & 16.13 \\
% & Gemini-Pro & 27.37 & 9.62 & 17.24 & 25.86 & 9.78 & 5.62 & 11.24 & 3.65 & \textbf{10.33} & \textbf{8.82} & 16.91 & 3.41 & 11.11 & 14.94 & 18.83 \\
% & Qwen-VL-Max & \textbf{37.89} & 17.31 & 24.14 & 30.03 & 16.87 & 7.87 & 18.54 & 6.15 & 8.10 & 5.88 & 21.32 & 2.65 & 12.75 & 20.73 & 26.27 \\
% & Qwen-VL-Plus & 10.53 & 11.54 & 3.45 & 10.49 & 3.45 & 0.00 & 2.43 & 0.00 & 2.96 & 2.94 & 8.82 & 1.68 & 4.84 & 5.79 & 8.31 \\
% \midrule
% \multirow{8}{*}{\makecell{Open-Source\\Image MLLMs}} & InternVL2-Llama3-76B & 17.89 & 15.38 & 13.79 & 24.43 & 13.79 & 1.12 & 8.71 & 1.12 & \textbf{9.56} & 0.00 & 9.80 & 0.00 & 12.90 & 10.36 & 15.32 \\
% & InternVL2-40B & 14.74 & \textbf{17.31} & \textbf{15.52} & 23.85 & \textbf{15.52} & 0.00 & 7.96 & 0.00 & 5.36 & 0.00 & 12.50 & 0.00 & 7.62 & 9.76 & 14.69 \\
% & InternVL2-8B & 13.68 & 13.46 & 8.62 & 18.25 & 4.04 & 0.00 & 7.43 & 0.00 & 3.04 & \textbf{5.88} & \textbf{18.63} & 2.45 & 3.16 & 8.23 & 13.27 \\
% & LLaVA-NEXT-72B & 16.84 & 3.85 & 10.34 & 20.26 & 10.34 & \textbf{3.37} & 8.61 & \textbf{3.37} & 6.46 & 2.94 & 12.01 & \textbf{2.94} & 11.25 & 8.54 & 12.65 \\
% & LLaVA-OneVision-72B & \textbf{27.37} & 15.38 & \textbf{15.52} & \textbf{28.30} & \textbf{15.52} & \textbf{3.37} & \textbf{10.77} & \textbf{3.37} & 6.21 & 2.94 & 11.03 & \textbf{2.94} & 4.76 & \textbf{14.33} & \textbf{19.44} \\
% & LLaVA-OneVision-7B & 16.84 & \textbf{17.31} & 5.17 & 9.05 & 3.28 & 1.12 & 8.15 & 0.80 & 3.36 & 2.94 & 9.80 & 1.68 & 9.35 & 9.14 & 12.45 \\
% & VILA-40B & 18.95 & 7.69 & 5.17 & 12.07 & 5.17 & 1.12 & 5.15 & 1.12 & 6.94 & 0.00 & 7.60 & 0.00 & \textbf{20.37} & 7.93 & 11.03 \\
% & VILA-8B & 15.79 & 9.62 & 1.72 & 8.91 & 0.96 & 0.00 & 3.46 & 0.00 & 3.98 & 2.94 & 6.37 & 1.68 & 3.42 & 6.71 & 9.27 \\
% \midrule
% \multirow{4}{*}{\makecell{Open-Source\\Video MLLMs}} & \makecell[l]{LLaVA-NeXT-Video-32B-Qwen} & 21.05 & 7.69 & 6.90 & 14.08 & 5.34 & 0.00 & \textbf{8.61} & 0.00 & \textbf{3.42} & 2.94 & \textbf{12.01} & 0.98 & 4.23 & 8.84 & 13.39 \\
% & LLaVA-Video-72B-Qwen2 & \textbf{27.37} & \textbf{9.62} & \textbf{15.52} & \textbf{24.28} & \textbf{9.62} & 1.12 & 8.05 & 0.86 & 2.84 & 0.00 & 9.80 & 0.00 & 7.02 & 12.50 & \textbf{16.95} \\
% & Oryx-34B & 18.95 & 3.85 & 5.17 & 13.07 & 4.89 & 1.12 & 7.02 & 1.00 & 2.65 & 0.00 & 8.33 & 0.00 & \textbf{9.09} & 7.32 & 11.33 \\
% & VideoLLaMA2-72B & \textbf{27.37} & \textbf{9.62} & 12.07 & 18.68 & 6.35 & \textbf{2.25} & 7.49 & \textbf{1.38} & 2.30 & \textbf{5.88} & 10.78 & \textbf{2.39} & 3.92 & \textbf{12.81} & 15.91 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[h!]
\centering
\vspace{-2em}
\captionsetup{skip=5pt}
\vspace{-0.5em}
\caption{Results Overview}
% \label{tab:main_results}
\renewcommand{\arraystretch}{1.3}
\scalebox{0.685}{
\begin{tabular}{lccccccccccccc cc}
\toprule
\multirow{2}{*}{\#Model} & \multicolumn{1}{>{\columncolor{AttrQAColor}}c}{Attr. QA} & \multicolumn{1}{>{\columncolor{SpatialQAColor}}c}{Spatial QA} & \multicolumn{3}{>{\columncolor{NavigationColor}}c}{Navigation} & \multicolumn{4}{>{\columncolor{ObjectInteractionColor}}c}{Object Interaction} & \multicolumn{4}{>{\columncolor{SocialInteractionColor}}c}{Social Interaction} & \multicolumn{2}{c}{\textbf{Overall}} \\
\cmidrule(r){2-3} \cmidrule(r){4-6} \cmidrule(r){7-10} \cmidrule(r){11-14} \cmidrule(r){15-16}
& Succ. & Succ. & Succ. & GcS & SPL & Succ. & GcS & SPL & Afford. & Succ. & GcS & SPL & Afford. & Succ. & GcS \\

\midrule
\multicolumn{16}{c}{\textit{Baseline}} \\
\midrule
\texttt{Random} & 11.58 & 7.69 & 3.45 & 8.76 & 3.45 & 0.00 & 6.18 & 0.00 & 2.54 & 2.94 & 8.33 & 2.94 & 3.44 & 5.49 & 8.66 \\
\texttt{Human} & 98.95 & 92.31 & 96.55 & 97.84 & 82.28 & 97.75 & 99.44 & 90.73 & 96.20 & 100.00 & 100.00 & 89.96 & 98.39 & 97.26 & 97.94 \\
\midrule
\multicolumn{16}{c}{\textit{Closed-Source Image MLLMs}} \\
\midrule
GPT-4o & 37.78 & \textbf{34.00} & \textbf{32.69} & \textbf{45.51} & \textbf{24.19} & \textbf{13.58} & \textbf{24.79} & \textbf{7.34} & 9.41 & 5.88 & 18.63 & \textbf{3.76} & 3.01 & \textbf{26.38} & \textbf{32.93} \\
GPT-4o-Mini & 31.58 & 15.38 & 27.59 & 39.51 & 15.34 & 2.25 & 17.42 & 1.50 & 9.18 & 5.88 & \textbf{22.06} & 2.98 & \textbf{16.99} & 17.68 & 25.58 \\
Gemini-Flash-1.5 & 26.32 & 13.46 & 5.17 & 17.10 & 3.51 & 2.25 & 7.58 & 0.96 & 10.00 & 2.94 & 12.50 & 1.47 & 4.92 & 11.59 & 16.13 \\
Gemini-Pro-1.5 & 27.08 & 9.62 & 16.67 & 25.00 & 9.46 & 5.49 & 11.36 & 3.57 & \textbf{10.33} & \textbf{8.82} & 16.91 & 3.41 & 11.11 & 14.71 & 18.64 \\
Qwen-VL-Max & \textbf{37.89} & 17.31 & 24.14 & 30.03 & 16.87 & 7.87 & 18.54 & 6.15 & 8.10 & 5.88 & 21.32 & 2.65 & 12.75 & 20.73 & 26.27 \\
Qwen-VL-Plus & 10.53 & 11.54 & 3.45 & 10.49 & 3.45 & 0.00 & 2.43 & 0.00 & 2.96 & 2.94 & 8.82 & 1.68 & 4.84 & 5.79 & 8.31 \\
\midrule
\multicolumn{16}{c}{\textit{Open-Source Image MLLMs}} \\
\midrule
InternVL2-Llama3-76B & 17.89 & 15.38 & 13.79 & 24.43 & 13.79 & 1.12 & 8.71 & 1.12 & \textbf{9.56} & 0.00 & 9.80 & 0.00 & 12.90 & 10.36 & 15.32 \\
InternVL2-40B & 14.74 & \textbf{17.31} & \textbf{15.52} & 23.85 & \textbf{15.52} & 0.00 & 7.96 & 0.00 & 5.36 & 0.00 & 12.50 & 0.00 & 7.62 & 9.76 & 14.69 \\
InternVL2-8B & 13.68 & 13.46 & 8.62 & 18.25 & 4.04 & 0.00 & 7.43 & 0.00 & 3.04 & \textbf{5.88} & \textbf{18.63} & 2.45 & 3.16 & 8.23 & 13.27 \\
LLaVA-NEXT-72B & 16.84 & 3.85 & 10.34 & 20.26 & 10.34 & \textbf{3.37} & 8.61 & \textbf{3.37} & 6.46 & 2.94 & 12.01 & \textbf{2.94} & 11.25 & 8.54 & 12.65 \\
LLaVA-OneVision-72B & \textbf{27.37} & 15.38 & \textbf{15.52} & \textbf{28.30} & \textbf{15.52} & \textbf{3.37} & \textbf{10.77} & \textbf{3.37} & 6.21 & 2.94 & 11.03 & \textbf{2.94} & 4.76 & \textbf{14.33} & \textbf{19.44} \\
LLaVA-OneVision-7B & 16.84 & \textbf{17.31} & 5.17 & 9.05 & 3.28 & 1.12 & 8.15 & 0.80 & 3.36 & 2.94 & 9.80 & 1.68 & 9.35 & 9.14 & 12.45 \\
VILA-40B & 18.95 & 7.69 & 5.17 & 12.07 & 5.17 & 1.12 & 5.15 & 1.12 & 6.94 & 0.00 & 7.60 & 0.00 & \textbf{20.37} & 7.93 & 11.03 \\
VILA-8B & 15.79 & 9.62 & 1.72 & 8.91 & 0.96 & 0.00 & 3.46 & 0.00 & 3.98 & 2.94 & 6.37 & 1.68 & 3.42 & 6.71 & 9.27 \\
\midrule
\multicolumn{16}{c}{\textit{Open-Source Video MLLMs}} \\
\midrule
LLaVA-NeXT-Video-32B-Qwen & 21.05 & 7.69 & 6.90 & 14.08 & 5.34 & 0.00 & \textbf{8.61} & 0.00 & \textbf{3.42} & 2.94 & \textbf{12.01} & 0.98 & 4.23 & 8.84 & 13.39 \\
LLaVA-Video-72B-Qwen2 & \textbf{27.37} & \textbf{9.62} & \textbf{15.52} & \textbf{24.28} & \textbf{9.62} & 1.12 & 8.05 & 0.86 & 2.84 & 0.00 & 9.80 & 0.00 & 7.02 & 12.50 & \textbf{16.95} \\
Oryx-34B & 18.95 & 3.85 & 5.17 & 13.07 & 4.89 & 1.12 & 7.02 & 1.00 & 2.65 & 0.00 & 8.33 & 0.00 & \textbf{9.09} & 7.32 & 11.33 \\
VideoLLaMA2-72B & \textbf{27.37} & \textbf{9.62} & 12.07 & 18.68 & 6.35 & \textbf{2.25} & 7.49 & \textbf{1.38} & 2.30 & \textbf{5.88} & 10.78 & \textbf{2.39} & 3.92 & \textbf{12.81} & 15.91 \\
\bottomrule
\end{tabular}%
}
% \vspace{-1.2em}
\end{table*}


% Qwen-VL-Max & \textbf{43.75} & 32.69 & \textbf{36.21} & \textbf{39.08} & \textbf{26.31} & 12.50 & 14.39 & 6.94 & 9.98 & 11.76 & 16.18 & 10.23 & 12.40 & 28.96 & 30.44 \\
% GPT-4o & 38.54 & \textbf{34.62} & 31.03 & 37.93 & 20.96 & \textbf{22.73} & \textbf{29.55} & \textbf{16.16} & 17.13 & \textbf{20.59} & \textbf{26.47} & \textbf{13.55} & 14.94 & \textbf{30.49} & \textbf{34.15} \\
% GPT-4o-Mini & 32.29 & 23.08 & 31.03 & 36.49 & 23.98 & 15.91 & 19.60 & 9.44 & 26.77 & 5.88 & 11.76 & 4.78 & 23.08 & 23.47 & 26.04 \\
% Qwen-VL-Plus & 17.71 & 13.46 & 5.17 & 6.61 & 4.60 & 0.00 & 1.89 & 0.00 & 4.92 & 0.00 & 0.00 & 0.00 & 22.22 & 8.23 & 8.99 \\
% Gemini-Flash ($t=0$) & 25.26 & 7.69 & 17.24 & 28.16 & 17.24 & 1.12 & 6.46 & 1.12 & 4.67 & 3.03 & 10.61 & 3.03 & 1.35 & 12.23 & 16.39 \\
% Gemini-Flash ($t>0$) & \textbf{28.42} & \textbf{15.38} & \textbf{10.34} & \textbf{22.56} & \textbf{10.34} & \textbf{6.74} & \textbf{21.07} & \textbf{6.74} & \textbf{11.22} & \textbf{11.76} & \textbf{28.43} & \textbf{11.76} & \textbf{12.27} & \textbf{15.55} & \textbf{23.32} \\
% InternVL2-40B ($t > 0$) & 20.00 & \textbf{19.23} & \textbf{15.52} & 22.70 & \textbf{15.52} & 1.12 & 8.93 & 1.12 & 6.67 & \textbf{2.94} & 11.76 & \textbf{2.94} & 8.85 & 12.19 & 16.50 \\
% InternVL2-Llama3-76B (($t=0$, prompt 2m) & 23.16 & 9.62 & 13.79 & 28.16 & 13.79 & 0.00 & 7.40 & 0.00 & 6.64 & 0.00 & 9.07 & 0.00 & 11.76 & 10.67 & 16.16 \\
% LLaVA-NEXT-72B ($t>0$) & 21.05 & 11.54 & 6.90 & 20.55 & 6.90 & 2.25 & 8.52 & 2.25 & 6.42 & 0.00 & \textbf{13.24} & 0.00 & 9.47 & 9.76 & 15.24 \\

% Gemini-Flash & 30.21 & 28.85 & 17.24 & 19.83 & 9.45 & 21.59 & 23.86 & 15.09 & 14.15 & 17.65 & 22.06 & 12.93 & \textbf{26.09} & 24.09 & 25.61 \\
% Gemini-Pro & 41.67 & 32.69 & 15.52 & 18.68 & 11.05 & 13.64 & 16.67 & 8.34 & \textbf{39.47} & 17.65 & 20.59 & 13.43 & 16.90 & 25.61 & 27.29 \\
% InternVL2-40B & 22.92 & 17.31 & 17.24 & 22.13 & 8.95 & 5.68 & 10.98 & 3.18 & 14.49 & 5.88 & 11.76 & 2.98 & 12.63 & 14.63 & 17.53 \\
% InternVL2-Llama3-76B & 20.83 & 21.15 & 13.79 & 19.83 & 8.11 & 3.41 & 5.11 & 2.00 & 9.44 & 2.94 & 4.41 & 2.94 & 13.89 & 13.11 & 14.78 \\
% LLaVA-NEXT-72B & 26.04 & 11.54 & \textbf{18.97} & \textbf{24.43} & \textbf{15.75} & \textbf{9.09} & \textbf{11.74} & \textbf{6.62} & 10.90 & \textbf{14.71} & \textbf{20.59} & \textbf{12.39} & 17.11 & 16.77 & 19.06 \\
% LLaVA-OneVision-72B & 29.17 & 21.15 & \textbf{18.97} & 22.99 & 15.47 & 3.41 & 8.71 & 2.73 & 10.81 & 8.82 & 13.24 & 5.43 & 19.28 & \textbf{17.07} & \textbf{19.67} \\
% VILA-40B & \textbf{35.42} & \textbf{26.92} & 1.72 & 4.31 & 1.72 & 3.41 & 5.68 & 3.41 & \textbf{15.66} & 5.88 & 8.82 & 5.88 & \textbf{19.75} & 16.46 & 17.83 \\
